Equipping Millimeter-Wave Full-Duplex with Analog Self-Interference Cancellation

There have been recent works on enabling in-band full-duplex operation using millimeter-wave (mmWave) transceivers. These works are based solely on creating sufficient isolation between a transceiver's transmitter and receiver via multiple-input multiple-output (MIMO) precoding and combining. In this work, we propose supplementing these beamforming strategies with analog self-interference cancellation (A-SIC). By leveraging A-SIC, a portion of the self-interference is cancelled without the need for beamforming, allowing for more optimal beamforming strategies to be used in serving users. We use simulation to demonstrate that even with finite resolution A-SIC solutions, there are significant gains to be had in sum spectral efficiency. With a single bit of A-SIC resolution, improvements over a beamforming-only design are present. With 8 bits of A-SIC resolution, our design nearly approaches that of ideal full-duplex operation. To the best of our knowledge, this is the first mmWave full-duplex design that combines both beamforming and A-SIC to achieve simultaneous transmission and reception in-band.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


***************************** Subdirectories ******************************

bibtex   - The IEEEtran BibTeX style package.

extras   - Supplementary material that may be of interest.

testflow - The testflow diagnostic suite for verifying PS/PDF output.

tools    - The IEEEtrantools.sty package which provides several commands
           from the IEEEtran.cls file for use with other LaTeX classes.


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex,
                   bare_jrnl.tex, bare_jrnl_comsoc.tex,
                   bare_jrnl_compsoc.tex, bare_jrnl_transmag.tex
***************************************************************************


==> sec-acknowledgement.tex <==
\section*{Acknowledgments}

We thank Arun Ghosh, Tom Novlan, Milap Majmundar, and Salam Akoum from AT\&T Labs for their insights.

==> sec-contribution-old.tex <==
\section{Proposed Design} \label{sec:contribution}

We now present an \asic design and \mimo precoding and combining designs that enable \fd operation at \mmwave by mitigating \si that would otherwise be incurred.

\subsection{Beamtraining}

Integral to our contribution is the fact that it is tailored for practical \mmwave systems using beamtraining. 

Channel estimation in \mmwave systems is often significantly different than that in sub-$6$ GHz systems due to the hybrid architecture frequently used. This is because \glspl{dac} at the transmitter and \glspl{adc} at the receiver are seen through the \rf beamformers, meaning the system cannot directly measure each antenna's observation. While there have been compressed sensing based solutions that leverage the spatial (angular) sparsity of the \mmwave channel (see \eqref{eq:desired-channel}), there are difficulties with practically implementing such strategies, especially given high path loss experienced at \mmwave. Compressed sensing based channel estimation relies on beam patterns that have poor directionality. Given the path loss experienced at \mmwave, this can clearly create problems in meeting sufficient link margin.

Given this, practical systems have instead turned to a more robust means of establishing a link without the need for prior channel knowledge. In beamtraining, time periods are allocated for a search to take place between \mmwave nodes. Often times, a sectorized search through a beamtraining codebook takes place whose output is a pair of \rf beamformers for a given link: one at the corresponding transmitter (i.e., \prerf) and one at the corresponding receiver (i.e., \comrf).

From here, we assume that beamtraining has taken place for communication from $k$ to $i$ and from $i$ to $j$. The beamtraining period provides selections for $\prerf\node{k}$ and $\comrf\node{i}$ as well as for $\prerf\node{i}$ and $\comrf\node{j}$. Our design does not rely on a specific selection process for beamtraining---whichever \rf beamformers are chosen, our design will design for.

With the \rf beamformers fixed, communication effectively reduces to conventional fully-digital \mimo, where the \glspl{dac} and \glspl{adc} have direct access to the \textit{effective channel} as seen through the \rf beamformers. We remark that channel estimation now becomes not only more straightforward but also much more reduced since channels that were once $\Nr \times \Nt$ are now merely $\Nrfrx \times \Nrftx$. In the design that follows, we	 will assume perfect channel estimation and full \gls{csir} and \gls{csit}.


\subsection{Analog SIC Design}
We consider the case where the \mmwave transceiver's \glspl{pa} and \glspl{lna} are linear. (Alternatively, we could assume that the transceiver's \glspl{pa} and \glspl{lna} are per \rf chain (rather than per antenna element).

\begin{align}
\channeltilde_{ii} \triangleq \comrf\ctransnode{i} \channel_{ii} \prerf\node{i}
\end{align}


\subsection{Precoding and Combining Design}
Having the \rf precoding and combining matrices fixed from beamtraining, our design will be in tailoring the baseband precoding and combining matrices to mitigate \si, enabling \fd operation.

We first consider the link from $i$ to $j$. In transmitting to $j$, $i$ will push some of its energy into the \si channel $\channel_{ii}$ which gets received by its own combiner.





==> sec-system-model-old.tex <==
\section{System Model} \label{sec:system-model}

%\begin{figure*}[!t]
%	% ensure that we have normalsize text
%	\normalsize
%	% Store the current equation number.
%	% \setcounter{mytempeqncnt}{\value{equation}}
%	% Set the equation number to one less than the one
%	% desired for the first equation here.
%	% The value here will have to changed if equations
%	% are added or removed prior to the place these
%	% equations are referenced in the main text.
%	% \setcounter{equation}{4}
%	\centering
%	\includegraphics[width=\linewidth]{fig/mmwave_hybrid_beamforming_block}
%	\caption{Hybrid analog/digital beamforming used by \mmwave systems.}
%	% Restore the current equation number.
%	% \setcounter{equation}{\value{mytempeqncnt}}
%	% IEEE uses as a separator
%	% \hrulefill
%	% The spacer can be tweaked to stop underfull vboxes.
%	\vspace*{4pt}
%\end{figure*}


% In our design, we consider the \mmwave network exhibited in \figref{fig:network}. 
%We assume node $i$ is a \fd transceiver capable of simultaneously realizing independent transmit and receive beamformers, while nodes $j$ and $k$ are \hd devices. 

In our design, we consider the \mmwave network shown in \figref{fig:network} comprised of three nodes: $i$, $j$, and $k$. Node $i$ is a \fd transceiver transmitting to $j$ while receiving from $k$ (in-band). Node $i$ has separate transmit and receive arrays meaning it is capable of simultaneously realizing independent transmit and receive beamformers. Nodes $j$ and $k$ are \hd devices. We remark that, together, $j$ and $k$ could represent another \fd device. We assume that all precoding and combining is done via fully-connected hybrid beamforming \cite{Heath_Gonzalez-Prelcic_Rangan_Roh_Sayeed_2016}, where the combination of baseband and \rf beamforming is used at each transmitter and receiver.

Let $\Nt\node{m}$ $(\Nr\node{m})$ be the number of transmit (receive) antennas at node $m \in \{i,j,k\}$. Let $\Nrftx\node{m}$ $(\Nrfrx\node{m})$ be the number of \rf chains at the transmitter (receiver) of node $m \in \{i,j,k\}$. 

For the desired channels $\channel_{ij}$ and $\channel_{ki}$, we use the model in \eqref{eq:desired-channel}, where the \mimo channel matrix between a node's transmit array and a different node's receive array as 
% The channel matrix between a one node's transmit array and another node's receive array can be written as
\begin{align}
\channel = \sqrt{\frac{\Nt \Nr}{\numrays \numclust}} \sum_{m=1}^{\numclust} \sum_{n=1}^{\numrays} \beta_{mn} \rxresponsevector(\aoa_{mn}) \txresponsevector\ctrans(\aod_{mn}), \label{eq:desired-channel}
\end{align}
where $\rxresponsevector(\aoa_{mn})$ and $\txresponsevector(\aod_{mn})$ are the receive and transmit array responses, respectively, for ray $n$ within cluster $m$, which has some \gls{aoa}, $\aoa_{mn}$, and \gls{aod}, $\aod_{mn}$ \cite{Heath_Gonzalez-Prelcic_Rangan_Roh_Sayeed_2016}. The total number of clusters is $\numclust$ and the number of rays per cluster is $\numrays$.
Each ray has a random gain $\beta_{mn} \sim \cgauss{0}{1}$.
% The coefficient outside the summations is used to ensure that $\ev{ \frobeniustwo{ \mat{H} }} = \Nt\Nr$. Note that we have considered a single angular dimension (e.g., azimuth) for the \glspl{aoa} and \glspl{aod} for simplicity and to agree with our use of \glspl{ula} in simulation.

\begin{figure*}[!t]
	% ensure that we have normalsize text
	\normalsize
	% Store the current equation number.
	% \setcounter{mytempeqncnt}{\value{equation}}
	% Set the equation number to one less than the one
	% desired for the first equation here.
	% The value here will have to changed if equations
	% are added or removed prior to the place these
	% equations are referenced in the main text.
	% \setcounter{equation}{4}
	\centering
	\includegraphics[width=0.85\linewidth]{fig/fdx3}
	\caption{A \fd \mmwave node $i$ transmitting to $j$ as it receives from $k$ in-band.}
	\label{fig:network}
	% Restore the current equation number.
	% \setcounter{equation}{\value{mytempeqncnt}}
	% IEEE uses as a separator
	% \hrulefill
	% The spacer can be tweaked to stop underfull vboxes.
	\vspace*{4pt}
\end{figure*}


For the \si channel at $i$, $\channel_{ii}$, we use the Rician summation shown in \eqref{eq:si-channel-rice}, where $\kappa$ is the Rician factor. The \gls{los} component $\channel^{\textrm{LOS}}_{ii}$ is based on the spherical-wave \mimo model in \cite{ipr-bfc-2019-globecom,spherical-wave-mimo}, reserving it due to space constraints. The \gls{nlos} component $\channel^{\textrm{NLOS}}_{ii}$ is based on the model in \eqref{eq:desired-channel}.
\input{eq-si-channel-rice.tex}
It is worthwhile to remark that the \si channel is not well-characterized for \mmwave \fd systems, meaning our model may not align well with practice. The channel in \eqref{eq:si-channel-rice} is often full-rank, though we do not rely on its particular channel structure in our design. We expect our design will translate well to other, more practically-sound \si channels.
\input{eq-si-channel-los.tex}

Let $\symbvec\node{m}$ be the $\Ns\node{m} \times 1$ symbol vector intended for node $m \in \{i,j,k\}$ where $\ev{\symbvec\node{m}\symbvec\ctransnode{m}} = \frac{1}{\Ns\node{m}}\mat{I}$
% It is assumed that the devices have proper support for the number of streams being communicated (i.e., sufficient number of \rf chains).
Let $\noisevec\node{m} \sim \cgauss{\mat{0}}{\noisevar \Rn}$ be a noise vector received by the receive array at node $m$, where we have assumed a common noise covariance matrix across nodes. Defining $\sigma^2$ as the noise variance and letting $\Rn = \mat{I}$ and $\Rs = \mat{I}$ provides a convenient formulation. 
For $m,n \in \{i,j,k\}$, we define the link \gls{snr} from node $m$ to node $n$ as 
\begin{align}
%\snr_{mn} = \frac{\Pt\node{m} \ G^2_{mn}}{\sigma^2_n}
% \snr_{mn} \triangleq \frac{\Pt\node{m} G^2_{mn}}{\sigma^2_n B}, 
\snr_{mn} \triangleq \frac{\Pt\node{m} G^2_{mn}}{\sigma^2}, 
\end{align}
where $\Pt\node{m}$ is the transmit power at $m$ and $G^2_{mn}$ is the large-scale power gain of the propagation from $m$ to $n$.  % Note that we have assumed a frequency-flat transmit power and large-scale gain indicating that the \gls{snr} (by our definition) is frequency-flat.

Let $\prebb\node{m}$ $(\combb\node{m})$ be the baseband precoding (combining) matrix at node $m \in \{i,j,k\}$. Let $\prerf\node{m}$ $(\comrf\node{m})$ be the \rf precoding (combining) matrix at $m \in \{i,j,k\}$. We impose a constant amplitude constraint on the entries of the \rf beamformers representing the fact that they have phase control and no amplitude control. Further, we assume the phase shifters have finite resolution, though our design does not rely on a particular resolution.

For the sake of analysis, we impose a uniform power allocation across streams. To do this, we normalize the baseband precoder for each stream such that 
\begin{align}
{\Big\Vert\prerf\node{m}\entry{\prebb\node{m}}{:,\ell}\Big\Vert_{\textsf{F}}}^2 = 1 \ \forall \ \ell \in [0,\Ns\node{m}-1]  % \frac{\Nt}{\Ns\node{m}}.
\end{align}
which ensures that for all $m \in \{i,j,k\}$
\begin{align}
\frobenius{\prerf\node{m}{\prebb\node{m}}}^2 = \Ns\node{m}.
\end{align}

\begin{figure*}[!t]
	% ensure that we have normalsize text
	\normalsize
	% Store the current equation number.
	\setcounter{mytempeqncnt}{\value{equation}}
	% Set the equation number to one less than the one
	% desired for the first equation here.
	% The value here will have to changed if equations
	% are added or removed prior to the place these
	% equations are referenced in the main text.
	\setcounter{equation}{4}
	\begin{align}
	\rxvec\node{i} = \ & \combb\ctransnode{i} \comrf\ctransnode{i} \left(\sqrt{\snr_{ki}} \  \channel_{ki} \prerf\node{k} \prebb\node{k} \symbvec\node{i}
	+ \sqrt{\snr_{ii}} \ \channel_{ii} \prerf\node{i} \prebb\node{i} \symbvec\node{j} + \noisevec\node{i} \right) \label{eq:est-i}
	\end{align}
	\begin{align}
	\rxvec\node{j} = \ & \combb\ctransnode{j} \comrf\ctransnode{j} \left(\sqrt{\snr_{ij}} \  \channel_{ij} \prerf\node{i} \prebb\node{i} \symbvec\node{j}
	+ \noisevec\node{j} \right) \label{eq:est-j}
	\end{align}
	% Restore the current equation number.
	\setcounter{equation}{\value{mytempeqncnt}}
	% IEEE uses as a separator
	\hrulefill
	% The spacer can be tweaked to stop underfull vboxes.
	\vspace*{4pt}
\end{figure*}

\addtocounter{equation}{1}

Recall that we are considering the network where $i$ is transmitting to $j$ while $i$ is receiving from $k$ (in a \fd fashion). A \mimo formulation gives us an estimated received symbol as \eqref{eq:est-i}.
Notice that the transmitted signal from $i$ intended for $j$ traverses through the \si channel $\channel_{ii}$ and is received by the combiner at $i$ being used for reception from $k$. 
The estimated receive symbol at $j$ from $i$ is \eqref{eq:est-j}, where $j$ does not encounter any \si since it is a \hd device. We ignore adjacent user interference between $j$ and $k$---justified by the high path loss and directionality at \mmwave.

